Stellar feedback impact on the ionized gas kinematics in the dwarf galaxy Sextans B

We investigated the ionised and atomic gas kinematics and excitation state in the central region of ongoing star formation of the nearby low-metallicity dwarf galaxy Sextans B. The analysis is based on the new observations performed in Ha emission line with high resolution ($R \sim 16000$) scanning Fabry-Perot interferometer at the 6-m BTA SAO RAS telescope, and on the long-slit spectral observations at the 9.2-m SALT and 2.5-m CMO SAI MSU telescopes. Strong non-circular gas motions detected in the studied regions probably resulted from the off-plane gas motions and impact of stellar feedback. We identified six regions of elevated Ha velocity dispersion, five of which exhibit asymmetric or two-component Ha line profiles. Three of these regions are young ($<1.1$ Myr) expanding ($V_{\rm exp} \sim 25-50\ {\rm km\ s^{-1}}$) superbubbles. We argue that at least three regions in the galaxy could be supernova remnants. We conclude that supernovae feedback is the dominant source of energy for superbubbles in Sextans B, which is expected for such a low metallicity, although we cannot rule out a strong impact of pre-supernova feedback for one superbubble.

==> SexB_intro_old.tex <==
Sextans B is a beatiful, very nearby and not well studied galaxy.

\red{Below is the Science Justification from the SALT proposal. We can use it as a starting point for introduction}

Understanding the feedback of stars on their environment is one
of the key problems in star and galaxy formation and evolution. Massive stars
are the main feedback agents influencing the surrounding interstellar medium (ISM) of galaxies
on both local and global scales. The ionizing radiation of OB stars, as well
as the kinetic energy of stellar winds and supernova explosions are heating the gas,
forming the cavities, shells,  ordered outflows and
chaotic turbulent motions in the gaseous disc of a galaxy.
The influence of multiple stellar winds and supernovae leads to
creation of the large superbubbles and shells with sizes up to several hundreds of parsecs.
Energy injected into the ISM by the ongoing star formation process is the main factor affecting
gas turbulent motions in dwarf galaxies (see Moiseev et al. 2015 and references therein).

Despite the well developed theoretical models of evolution of superbubbles (see, e.g.,
Weaver et al. 1977; Krause et al. 2013), a number of problems arise when one compares them
with observations. Among them are discrepancy between predicted and observed sizes and
energetics of superbubbles, in particular in the case of non-uniform medium
(see, e.g., Oey 2009 for review). Often these discrepancies have been solved assuming
a small filling-factor of ISM and low efficiency of mechanical energy transferring from
stars (e.g., Vasiliev et al. 2015, Yadav et al. 2017),
but the observational studies of evolution of superbubbles are necessary to completely understand 
the reasons of the discrepancies.
A low-metallicity environment in nearby dwarf galaxies is of especial interest for such studies.
Radiative loses are low there, and hence we may expect high mechanical energy of superbubbles
resulted as stellar feedback influence onto the ISM.
Even a single WR star might be crucial in evolution of ISM in very low metallicity systems
(see, e.g. Kehrig et al. 2016, 2018). 

High spectral and spatial resolution is crucial for identification of expanding ionized
structures in ISM of galaxies.
They reveal a multi-component emission line profiles in the spectra or demonstrate significantly 
enhanced velocity dispersion. Abilities of a scanning Fabry-Perot interferometer (FPI)
at the 6m Russian telescope providing both high spectral and spatial resolution allowed
our team to detect  several dozens of expanding superbubbles and giant supershells
in nearby dwarf galaxies (see, e.g., Egorov et al. 2018 and references therein). Most of the 
detected objects are related to young stellar clusters located inside them, however there are also 
observed some structures without any central driving sources with enough mechanical energy output to 
drive their expansion (e.g., Egorov et al. 2014, 2016). Beside the superbubbles around young massive 
clusters the individual stellar objects highly influencing to the ISM (supernovae remnants, WR and 
LBV stars) might be identified based on the analysis of the ionized gas velocity dispersion from FPI 
data (Moiseev \& Lozinskaya 2012), but the spectral observation are necessary to reveal their 
nature.

Recently we observed the nearby low-metallicity galaxy Sextans B with FPI in H$\alpha$ emission 
line at the Russian 6-m telescope (see Figures 1-3).
This galaxy is of particular interest because it is a closest (1.4 Mpc) isolated dwarf galaxy 
without any massive companion. Hence it is a perfect laboratory for study the feedback processes 
with free of the contamination by significant external interactions, and the proximity of the galaxy 
allow us to analyse the interaction between massive stars and ISM with high spatial resolution. An 
analysis of the obtained FPI data uncovered 5 regions (4 HII regions and one point-like source) of 
significantly
enhanced velocity dispersion of ionized gas; all of them demonstrate multicomponent or asymmetrical 
line profile. Based on the obtained data we estimated the unusually high expansion velocities (up to 
100 km/s, in comparison with 20-30 km/s typically observed in other dIrr galaxies) of the observed 
superbubbles (See Figures 2 and 3). In terms of classical model of the evolution of superbubbles around star clusters
driven by multiple stellar winds and supernovae it lead to the very low kinematical age (less than 
0.3 Myr). Alternatively, studied objects could be supernovae remnants, WR stars with high-velocity 
wind, or other types of high-energy objects influencing on the ISM. Thus, Sextans B appears to be 
very intriguing galaxy providing an opportunity to study the interaction between massive stars and 
ISM in low-metallicity environment for 5 unique emission objects with observed high velocities 
simultaneously. High quality spectral observations of these regions are needed to uncover their 
nature. 

The  galaxy was observed previously twice with long-slit spectrographs at NTT (Kniazev et al., 2005) 
and VLT (Magrini et al., 2005), but only one of the objects of interest (\#1 in our list) was 
crossed by the slits. Unfortunately, because of very low signal-to-noise ratio at the NTT spectra 
for this object, we are unable to use it for the analysis.


\red{Below are some citations extracted by TA from various literature that can be useful here}


"Today it is clear that dwarf galaxies sustain a high SF efficiency over several hundred Myr, and even up to 1000~Myr in some cases \citep{Mcquinn2009, Mcquinn2010a, Mcquinn2010b} with local short starbursts occurring during this period."

In this work we focus on the dIrr galaxy  Sextans B (DDO 70); RA=10h00m00s, D=+5d19m56s.
Its distance has been determined to be 1.32 Mpc (a distance modulus $25.61\pm 0.27$)
 ( van den Bergh, Ap.J. 517, L97-L99, 1999;  S. Sakai, B.F. Madore, W.L.Freedman, 1997, AJ,480,589).
The galaxy is located in  close proximity to Sextans A, NGC 3109 and the Antlia dwarf.
According to modern understanding (see Magrini et al, 2002 and references therein)  these dIrr galaxies form a physical
associated group lying just outsede the outskirt of the Local Group  [ S. van den Bergh, ApJ 517, L97 (1999); R.B. Tully, R.S. Sommerville,
N. Trentham, M.A. Verheijen, ApJ 569, 573 (2002)].  Therefore it would be the nearest association outside the
LG (van den Bergh S., 2000, in The Galaxies of the Local Group, Cambridge University Press, 269).
According to Magrini et al (2002)  these galaxies are  interesting because they
represent a group of dwarf galaxies relatively isolated from giant
galaxies. The stellar population of Sextans B "is dominated
by red giants (Sakai et al. 1997), with a prominent contribution
of intermediate-age asymptotic branch stars. A
young population is also present, indicating a complex,
low-rate and likely discontinuous star formation throughout
the galaxy lifetime (Tosi et al. 1991; van den Bergh
2000). According to M. Tosí, L. Greggio, G. Marconi, and P. Focardi, AJ 102,951,1991,
the star formation in the galaxy "is likely to have proceeded in long
periods of quiet activity separated by short quiescent intervals,
and it is not necessarily active now."

    A dozen HII regions are known (Strobel et al.
1991); 5 PNe have been identified (Magrini et al, 2002) in the galaxy.

------------------
Abstract Magrini et al, 2002:
"The Local Group Census: Planetary nebulae in Sextans B?"
L. Magrini, R. L. M. Corradi, N. A. Walton, A. A. Zijlstra, D. L. Pollacco,
J. R. Walsh, M. Perinotto, D. J. Lennon, and R. Greimel.

Abstract. Five planetary nebulae (PNe) have been discovered in the nearby dwarf irregular galaxy.
 Emission line images were obtained using the Wide Field Camera of the 2.5 m Isaac Newton Telescope (INT) at La Palma
 (Spain). The candidate PNe were identified by their point-like appearance and relatively strong [O iii] emission-line
 fluxes. They are located within a galactocentric distance of 2.8 arcmin, corresponding to 1.1 kpc at the distance of
 Sextans B. Luminosities are in the range 1800-5600 L(sol). Sextans B is one of the smallest dwarf irregular galaxies
with a PN population. The number of PNe detected suggest an enhanced star formation rate between 1 and 5 Gyr ago."


---------------------

=====================================================













Из работы Sextans A B-2005: 

L. Magrini, P. Leisy, R. L. M. Corradi, M. Perinotto, A. Mampaso, and J. M. Vílchez,
A.Ap. 443, 115–132 (2005)
"The chemistry of planetary nebulae and HII regions in the dwarf galaxies Sextans A and B from deep VLT spectra."
    (у меня Sextans A B-2005)


ABSTRACT
Spectroscopic observations obtained with the VLT of one planetary nebula (PN) in Sextans A and of five PNe in Sextans B and of several
HII regions in these two dwarf irregular galaxies are presented. The extended spectral coverage, from 320.0 to 1000.0 nm, and the large
telescope aperture allowed us to detect a number of emission lines, covering more than one ionization stage for several elements (He, O,
S, Ar). The electron temperature diagnostic [O III] line at 436.3 nm was measured in all six PNe and in several HII
 regions allowing for an accurate determination of the ionic and total chemical abundances by means of the Ionization Correction Factors method. For the time
being, these PNe are the farthest ones where such a direct measurement of the electron temperature is obtained.
In addition, all PNe and HII regions were also modelled using the photoionization code
 CLOUDY (Ferland et al. 1998, PASP, 110, 761). The physico-chemical properties of PNe and HII regions are presented
 and discussed. A small dispersion in the oxygen abundance of HII regions was found in both galaxies:
12 + log (O/H) = 7.6 ± 0.2 in Sextans A, and 7.8 ± 0.2 in Sextans B. For the five PNe of Sextans B, we find
that 12 + log (O/H) = 8.0 ± 0.3, with a mean abundance consistent with that of HII regions. The only PN known in
 Sextans A appears to have been produced by a quite massive progenitor, and has a significant nitrogen overabundance.
 In addition, its oxygen abundance is 0.4 dex larger than the mean abundance of HII
regions, possibly indicating an efficient third dredge-up for massive, low-metallicity PN progenitors.
 The metal enrichment of both galaxies is analyzed using these new data.


Из введения  этой работы

"Sextans A and Sextans B have approximately
the same V luminosity and located at a very similar distance
(1.3 Mpc, Dolphin et al. 2003 for Sextans A and 1.32 Mpc  for
Sextans B, van den Bergh, Ap.J. 517, L97-L99, 1999). Their separation in the sky (10.4 degrees) corresponds to about 280 kpc at the
adopted distance and their velocity difference is only
$23 \pm 6 \kms$. All these properties suggest a common formation
for these two galaxies, probably together with NGC 3109
and the Antlia galaxy, also at a similar distance and location
in the sky. Considering the mean distance of the four galaxies
from the barycentre of the Local Group (LG), 1.7 Mpc, this
sub-group is located beyond the zero velocity surface of the LG
(cf. vdB00) and can be considered the nearest external group of
galaxies. Then these galaxies are particularly interesting as they
represent a group of dwarf galaxies relatively isolated from giant
galaxies."


"The brightest HII regions of Sextans B were first catalogued
by Hodge (1974). Strobel et al. (1991) classified twelve
HII regions, whereas oxygen abundance was derived for four HII regions by Skillman et al. (1989).
Note, however, that these
spectroscopic studies were generally not deep enough (except
for one or two objects) to allow direct measurement of the nebular
electron temperature via detection of the [OIII] 436.3 nm
line, causing an important source of uncertainty in the determination
of their chemical abundances."


"Sextans B exhibits a very strong star formation at recent and intermediate ages (1–4 Gyrs ago), together with a very old population (cf. Mateo 1998). The different numbers of PNe,
 5 in Sextans B vs. 1 in Sextans A, was interpreted by Magrini et al. (2002) to be consistent with the different star formation histories of
the two galaxies for the age range covered by the PN progenitors,
Sextans B showing a stronger star formation rate than
Sextans A during the past 2–10 Gyrs."

"The high resolution WHT spectra allowed us to measure
the Doppler shift of the \OIII doublet lines, and in one case
also of \Hb, in three PNe of Sextans~B, namely PN 1, PN 4 and
PN 5. The heliocentric radial velocities are listed in Table 2.
They are consistent, within the errors, with the heliocentric radial
velocity of Sextans B ($300 \kms$ from NED) and with the
HI observations by Huchtmeier et al. (2003)."


``We find that the central stars of Sex B PNe had initial masses between
0.9 and 1.5 $M\odot$. Stars with these masses and with an
initial metallicity Z = 0.001 were born between about 10 and 2 Gyr ago (cf. Charbonnel et al. 1999, 1996).   As the mean oxygen
abundance of PNe in Sextans B is equal, within the errors,
to that of HII regions, this would mean that no noticeable
chemical enrichment has occurred in the galaxy since long time ago.''

``A recent very work about spectroscopy of H regions
and PNe of Sextans A and Sextans B is by Kniazev et al.
(2005). The authors derived chemical abundances of the PN
and of three HII regions in Sextans A, and of one PN (PN3)
and three HII regions in Sextans B with the ICF method. In
Sextans A, they found an oxygen abundance of $8.02\pm0.05$
in the PN and $7.54\pm0.06$ in three \HII regions, that, we
did not observe. These \HII regions belong to the same complex
of HSK14, HSK16, and HSK19, for which we derived
a mean 12 + log O/H= $7.65 \pm 0.1$. In PN3 of Sextans B they
 derived 12+log O/H= $7.47\pm0.16$, in agreement with our value
$7.5 \pm 0.2$. They also observed the same HII regions for which
we derived chemical abundances with the ICF method, SHK1,                                      I
SHK2, SHK5, finding 12 + log O/H = $7.50 \pm 0.08$, $7.55 \pm 0.06$,
$7.84 \pm 0.05$, respectively. These values are similar to our.''




Распределение \HI в галактиках  Sextans А и  Sextans В  детально исследовано (см. Skillman, Terlevich, Teuben, van Woerden, A.Ap. 198, 33-42, 1988;
S.D. VAN DYK, D. PUCHE, T. WONG, AJ, 116,2341-2362, 1998
E.M.Wilcots, D.A.Hunter, AJ, 123, 1476-1487,2002;
D.G.Barnes and W.J.G.de Blok, MNRAS, 351, 333-338, 2004;
D.A.Hunter, F.Zahedy, E.C. Bowsher,E.M. Wilcots, A. A. Kepley, and V. Gaal, AJ, 142-173, 2011;
B. Namumba, C. Carignan, and S. Passmoor, 2018 (у меня Sext A B-HI-2018)
и ссылки в этих работах.)

абстракт последней работы:
``Hi observations of Sextans A and B with the SKA
pathfinder KAT-7.''
B. Namumba, C. Carignan and S. Passmoor.
    ABSTRACT
“HI observations of the Local Group dwarf irregular galaxies Sextans A and B, obtained with the Karoo Array Telescope (KAT-7) are presented. The KAT-7 wide field of view and excellent surface brightness sensitivity allows us to verify the true HI extent of the galaxies. We derive HI extends of 30’ and 20’ and total HI fluxes of
$181 \pm 2.0 Jy.km.s^{-1}$ and $105 \pm 1.4$ Jy.km.s for Sextans A and B respectively. This result shows clearly the overestimate of the \HI extent and total flux of 54’ and $264 Jy.km. s^{-1}$ reported for Sextans A using the Effelsberg observations. Tilted ring models
allow us to derive the rotation curves (RCs) of Sextans A and B out to 550'' (~ 3.5kpc) and 650'' (~ 4 kpc) respectively. The RCs of the two galaxies are seen to decline in the outer parts. The dark matter distribution in Sextans A is better described by the pseudo-isothermal halo model when a M/L ratio of 0.2 is used. For Sextans B, the
mass model fits are not as good but again an isothermal sphere with a M/L of 0.2 represents best the data. Using the MOdified Newtonian Dynamics (MOND), better fits are obtained when the constant a0 is allowed to vary. The critical densities for gravitational instabilities are calculated using the Toomre-Q and cloud-growth based on shear criterion. We find that in regions of star formation, the cloud growth criterion based on shear explains better the star formation in both Sextans A and B.”

Рис 5 из этой работы:  Integrated Hi column density map of Sextans B superposed on a DSS image. Не эффектный.

          ---------------=============================================
В работе Steven R. Warren, Edward Molter, John M. Cannon, Alberto D. Bolatto, E.A.K. Adams,
Elijah Z. Bernstein-Cooper, Riccardo Giovanelli, Martha P. Haynes, Rodrigo Herrera-Camus, Katie Jameson,
Kristen B. W. McQuinn, Katherine L. Rhode, John J. Salzer, and Evan D. Skillman, ApJ, 814,30,2015 искали и не нашли СО эмиссию в Sextans A и Sextans В.
-------------------------------------------------------


------------------

ОЧЕНЬ ХОРОШИЕ картинки распределения оптического, H-alpha,  HI




    Из работы Sextans B-2007
"A globular cluster in the dwarf galaxy Sextans B"
M. E. Sharina, T. H. Puzia and A. S. Krylatyh

ABSTRACT:
We present spectroscopic observations of a massive globular cluster in the dwarf irregular galaxy Sextans B, discovered by us on Hubble Space Telescope Wide Field and Planetary Camera 2 (HST WFPC2) images. Long-slit spectra were obtained with the SCORPIO spectrograph on the the 6-m telescope ...
 We determine age, metallicity and alpha-element abundance ratio for
the globular cluster to be $2\pm1$ Gyr,$-1.35\pm0.25$ dex, and $0.1\pm0.1$ dex, respectively. Main photometric and structural parameters of it were determined using our surface photometry on the HST images.      The mass (~$10^5$ Msol), luminosity and structural parameters appear to
be typical for the globular clusters in our own Galaxy. Our findings shed a new light on the evolutionary history of Sextans B."

Использовать  из ВВЕДЕНИЯ:
"Sextans B is a rather isolated dwarf irregular galaxy, a member of the Antlia-Sextans group near the Local group [6, 7]. It is a faint galaxy, typical for the population of the Local Group and other nearby poor groups. Its central surface brightness in the filter B of the wide-band
Johnson-Cousins system is 22.8±0.2 mag/sq.sec.
The absolute blue magnitude, MB = -13.97, corresponds to the distance 1360 ± 70 kpc [9].
The chemical composition of HII regions and of planetary nebulae in the galaxy were extensively studied by many authors [10-13]. The star formation history of Sextans B according to stellar photometry studies was rather complex. According to [14-16] the galaxy experienced a powerful early star formation burst during the first 1-2 Gyr, and an    inсreased SF activity in the last 1-2 Gyr. Dolphin et al. [17] consider the star formation to be active during the whole life of the
galaxy. However, all the authors mention that the available
color-magnitude diagrams (CMDs) are not very deep to determine the age of the galaxy with an accuracy of ~ 2 - 3 Gyr. Kniazev and co-authors [13] discovered that one \HII region in the galaxy is twice as metal-rich in comparison to others. This implies considerable inhomogeneity in the present-day metallicity distribution in Sextans B.
In this paper we report for the first time the discovery and a detailed spectroscopic investigation of a GC in Sentans B with the SCORPIO spectrograph at the SAO RAS 6m telescope.


=======================


ИЗ Работы  AJ, 130, 1558-1573, 2005 

"SPECTROPHOTOMETRY OF SEXTANS A AND B: CHEMICAL ABUNDANCES OF HII REGIONS AND PLANETARY NEBULAE"
Alexei Y. Kniazev, Eva K. Grebel, Simon A. Pustilnik, Alexander G. Pramskij and Daniel B. Zucker

ABSTRACT
"We present the results of high-quality long-slit spectroscopy of planetary nebulae (PNe) and HII regions in the two dwarf irregular (dIrr) galaxies Sextans A and B, which belong to a small group of galaxies just outside the Local Group. The observations were obtained with the New Technology Telescope ESO Multi-Mode Instrument.
In Sextans A we obtained the element abundances in its only known PN and in three HII  regions with the classical Te method. The oxygen abundances in these three HII regions of Sextans A are all consistent within the individual rms uncertainties, with an average 12 + log (O/H) = $7.54 \pm 0.06$. The oxygen abundance of the PN in Sextans A is, however, significantly higher: 12 + log (O/H) = $8.02 \pm 0.05$. This PN is even more enriched in nitrogen and helium, suggesting a classification as a PN of type I. The PN abundances of S and Ar, which are presumably unaffected
by nucleosynthesis in the progenitor star, are well below those in the HII regions, indicating lower metallicity at the epoch of the PN progenitor formation (~1.5 Gyr ago, according to our estimates based on the PN parameters). In Sextans B we obtained spectra of one PN and six   HII regions. Element abundances with the Te method could be
derived for the PN and three of the HII regions. For two of these HII regions, which have a separation of only ~70 pc
in projection, the oxygen abundances do not differ within the rms uncertainties, with a mean of 12 + log (O/H) = 7.53 pm 0.05.   The third HII region, which is about 0.6 kpc northeast of the first two, is twice as metal-rich, with 12 + log (O/H) = 7.84 pm 0.05. This suggests considerable inhomogeneity in the present-day metallicity distribution
in Sextans B. Whether this implies a general chemical inhomogeneity among populations of comparable age in Sextans B, and thus a metallicity spread at a given age, or whether we happen to see the short-lived effects of
freshly ejected nucleosynthesis products prior to their dispersal and mixing with the ambient interstellar medium will require further study. For the PN we measured an O/H ratio of 12 + log (O/H) = 7.47 pm 0.16, consistent with that of the low-metallicity H II regions. We discuss the new metallicity data for the HII regions and PNe in the context of
the published star formation histories and published abundances of the two dIrr galaxies. Both dIrrs show generally similar star formation histories in the sense of continuous star formation with amplitude variations but differ in their detailed enrichment timescales and star formation rates as a function of time. If we combine the photometrically
derived estimates for the mean metallicity of the old red giant branch population in both dIrrs with the present-day metallicity of the HII regions, both dIrrs have experienced chemical enrichment by at least 0.8 dex ( lower limit) throughout their history."

ИЗ SUMMARY:

 3. In Sextans B one HII region (HII 5) is significantly enriched,
with an excess in O, N, S, and Ar of a factor of 2.5 pm 0.5
relative to the mean value of the two other H ii regions studied
here. This is strong evidence for chemical inhomogeneity in a
dIrr galaxy. Whether this implies a general chemical inhomogeneity
among populations of comparable age in Sextans B, and thus
a metallicity spread at a given age, or whether we happen to see
the short-lived effects of freshly ejected nucleosynthesis products
prior to their dispersal and mixing with the ambient ISM
will require further study.


5. The element abundances of PN3 in Sextans B are consistent
with those of the two HII regions with low metallicity. Comparison
of the element abundances for this PN and the two nearby
HII regions implies that the maximum O and N enrichment during
the last few gigayears (the estimated age of the progenitor
star of PN3) did not exceed ~0.4 dex.
